Does Recursive Knowledge Construction Help Agents Verify Consensus Claims in Science?

Recent scientific agents build knowledge recursively by retrieving evidence, constructing an intermediate state, and judging whether that state contains sufficient information. These agents are evaluated end-to-end, usually without ground truth, so the effect of each design choice is unknown. Here, we examined two design axes: (1) what the recursion builds (the state of evidence) and (2) what controls it (the judge that decides when to stop). To measure them, we defined consensus scientific claim verification and measured these effects on this task, where a system must establish a claim's consensus stance from the open literature. We built a new consensus claim dataset, ProClaim-eval, including 718 claims with SUPPORT and REFUTE gold labels from five expert-curated databases spanning molecular biology, nuclear physics, and astronomy. Our instrument, ProClaim, persists an evidence state outside the model's context, so each axis can be studied with the other held fixed. Against verification systems and general-purpose agent harnesses, ProClaim ranks among the top three, with a significant advantage over the harnesses. We found that the evidence state improves performance over in-context accumulation, and it also matters what is stored in it. In addition, a trained judge that reads the evidence state performs better than fixed-round stopping. A judge trained separately and never exposed to ProClaim-eval achieves the highest agreement with the gold labels on three of five subsets, where it matches the off-the-shelf Claude Sonnet~4.6 judge and outperforms Claude Haiku~4.5. Our results support recursively maintaining a structured evidence state outside the model's context as an effective design for verifying claims in scientific agents.

==> figs/fig_claim_diversity_table_caption.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/fig_claim_diversity_table.pdf}
\caption{\textbf{Claim diversity in the extended ProClaim-eval benchmark.}
One example claim per subset, verbatim from the released files, with the subset's claim count
(\textsc{support} / \textsc{refute} split) and the example's own gold label. Evaluation is
restricted to claims with a \textsc{support} or \textsc{refute} gold label (718 claims;
403 \textsc{support}, 315 \textsc{refute}); models nonetheless choose among three verdicts, with
\textsc{uncertain} serving only as an abstention. The five subsets instantiate five distinct
single-sentence templates over three scientific domains: molecular biology (ConnectomeDB,
SIGNOR, ExTRI), astronomy (NASA Exoplanet Archive) and nuclear physics (NUBASE).}
\label{fig:claim-diversity}
\end{figure}


==> figs/fig_rkc_overview_caption.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/fig_rkc_overview.pdf}
\caption{\textbf{Recursive knowledge construction and the two design axes this paper isolates.}
\textbf{(a)} A verifier turns a claim $c$ into a verdict by repeating retrieve--extract--judge over an
explicit evidence state $s_t$. The update step writes into the state; both the next retrieval and the
stopping decision read from it, which is what makes the loop recursive rather than a fixed pipeline:
round $t{+}1$ is a function of what round $t$ established. The loop halts at the first round $T$ where
the judge returns \textsc{stop}, and the verdict is read off the final state, so a claim is answered
\textsc{support} or \textsc{refute} only when the accumulated literature evidence settles it, and is
abstained on otherwise.
\textbf{(b)} The first component, the evidence state: retrieved papers, verbatim facts carrying a
\textsc{support}/\textsc{refute}/\textsc{neutral} stance and a link to their source paper, detected
conflicts, open sub-claims and the sufficiency history. It is persisted as JSON outside the model
context and reached through code, so its content is not compressed or paraphrased as rounds accumulate
(facts shown are illustrative).
\textbf{(c)} The second component, the stopping judge: per-paper features are pooled into a 24-dimensional
state representation and mapped by an MLP to a sufficiency score $\sigma(c,s_t)$, which stops the
recursion once it reaches $\delta=0.8$; a cap of $T_{\max}=4$ rounds bounds the run.
Shaded bands name the experimental manipulation of each component. Section~\ref{sec:exp_state} varies
what the recursion builds with the judge held fixed, and Section~\ref{sec:exp_judge} varies what controls
it with the state held fixed, so each axis is measured with the other unchanged.}
\label{fig:rkc_overview}
\end{figure}


==> tables/baseline_cost_main.tex <==
\begin{tabular}{@{} l | c | c @{}}
\toprule
  & \multicolumn{1}{c|}{\cellcolor{headerteal}\textbf{SIGNOR}} & \multicolumn{1}{c}{\cellcolor{headerlavender}\textbf{ConnectomeDB}} \\
\textbf{Method} & Cost (USD)$\downarrow$ & Cost (USD)$\downarrow$ \\
\midrule
Random & \underline{0.000} {\scriptsize$\pm$ 0.000} & \underline{0.000} {\scriptsize$\pm$ 0.000} \\
\midrule
\multicolumn{3}{@{}l}{\textit{LLM Only}} \\[2pt]
Claude Sonnet 4.6 & 0.002 {\scriptsize$\pm$ 0.000} & 0.003 {\scriptsize$\pm$ 0.000} \\
Gemini 2.5 Flash & 0.000 {\scriptsize$\pm$ 0.000} & 0.000 {\scriptsize$\pm$ 0.000} \\
\midrule
\multicolumn{3}{@{}l}{\textit{Static Retrieval S2 Top 5}} \\[2pt]
Claude Sonnet 4.6 & 0.009 {\scriptsize$\pm$ 0.000} & 0.010 {\scriptsize$\pm$ 0.000} \\
Gemini 2.5 Flash & 0.001 {\scriptsize$\pm$ 0.000} & 0.001 {\scriptsize$\pm$ 0.000} \\
\midrule
\multicolumn{3}{@{}l}{\textit{Static Retrieval Web Top 5}} \\[2pt]
Claude Sonnet 4.6 & 0.005 {\scriptsize$\pm$ 0.000} & 0.005 {\scriptsize$\pm$ 0.000} \\
Gemini 2.5 Flash & 0.000 {\scriptsize$\pm$ 0.000} & 0.000 {\scriptsize$\pm$ 0.000} \\
\midrule
\multicolumn{3}{@{}l}{\textit{Adaptive Retrieval}} \\[2pt]
ReAct + S2 & 0.273 {\scriptsize$\pm$ 0.000} & 0.263 {\scriptsize$\pm$ 0.003} \\
ReAct + Web & 0.077 {\scriptsize$\pm$ 0.000} & 0.088 {\scriptsize$\pm$ 0.002} \\
FIRE & 0.015 {\scriptsize$\pm$ 0.000} & 0.016 {\scriptsize$\pm$ 0.000} \\
SAFE & 0.038 {\scriptsize$\pm$ 0.001} & 0.042 {\scriptsize$\pm$ 0.001} \\
OpenScholar + S2 & 0.041 {\scriptsize$\pm$ 0.000} & 0.063 {\scriptsize$\pm$ 0.011} \\
\midrule
\textbf{ProClaim} (uncached, single run) & 2.248 & 1.834 \\
\textbf{ProClaim} (ours, cached) & 0.642 {\scriptsize$\pm$ 0.016} & 0.664 {\scriptsize$\pm$ 0.012} \\
\bottomrule
\end{tabular}


==> tables/baseline_metrics_aggregated_signor+connectomedb_se.tex <==
\begin{tabular}{@{} l | c c c c @{}}
\toprule
  & \multicolumn{4}{c}{\cellcolor{headerteal}\textbf{ProClaim-eval}} \\
\textbf{Method} & Agreement$\uparrow$ & $\boldsymbol{\Delta}\uparrow$ & FPR$\downarrow$ & FNR$\downarrow$ \\
\midrule
Random & 0.34 {\scriptsize$\pm$ 0.01} & \cellcolor{deltaxl}+0.41 & 0.33 {\scriptsize$\pm$ 0.00} & 0.65 {\scriptsize$\pm$ 0.01} \\
\midrule
\multicolumn{5}{@{}l}{\textit{LLM Only}} \\[2pt]
Claude Sonnet 4.6 & 0.54 {\scriptsize$\pm$ 0.00} & \cellcolor{deltal}+0.21 & 0.22 {\scriptsize$\pm$ 0.00} & 0.47 {\scriptsize$\pm$ 0.01} \\
Gemini 2.5 Flash & 0.57 {\scriptsize$\pm$ 0.00} & \cellcolor{deltam}+0.18 & 0.21 {\scriptsize$\pm$ 0.00} & 0.42 {\scriptsize$\pm$ 0.01} \\
\midrule
\multicolumn{5}{@{}l}{\textit{Static Retrieval S2 Top 5}} \\[2pt]
Claude Sonnet 4.6 & 0.51 {\scriptsize$\pm$ 0.00} & \cellcolor{deltal}+0.24 & 0.26 {\scriptsize$\pm$ 0.00} & 0.59 {\scriptsize$\pm$ 0.00} \\
Gemini 2.5 Flash & 0.53 {\scriptsize$\pm$ 0.00} & \cellcolor{deltal}+0.22 & 0.27 {\scriptsize$\pm$ 0.00} & 0.58 {\scriptsize$\pm$ 0.00} \\
\midrule
\multicolumn{5}{@{}l}{\textit{Static Retrieval Web Top 5}} \\[2pt]
Claude Sonnet 4.6 & 0.49 {\scriptsize$\pm$ 0.01} & \cellcolor{deltal}+0.26 & 0.24 {\scriptsize$\pm$ 0.00} & 0.63 {\scriptsize$\pm$ 0.01} \\
Gemini 2.5 Flash & 0.58 {\scriptsize$\pm$ 0.01} & \cellcolor{deltam}+0.17 & 0.24 {\scriptsize$\pm$ 0.00} & 0.59 {\scriptsize$\pm$ 0.00} \\
\midrule
\multicolumn{5}{@{}l}{\textit{Adaptive Retrieval}} \\[2pt]
ReAct + S2 & 0.62 {\scriptsize$\pm$ 0.01} & \cellcolor{deltam}+0.13 & 0.19 {\scriptsize$\pm$ 0.00} & 0.44 {\scriptsize$\pm$ 0.01} \\
ReAct + Web & 0.69 {\scriptsize$\pm$ 0.00} & \cellcolor{deltas}+0.07 & 0.16 {\scriptsize$\pm$ 0.00} & \underline{0.32} {\scriptsize$\pm$ 0.02} \\
FIRE & 0.62 {\scriptsize$\pm$ 0.00} & \cellcolor{deltam}+0.13 & 0.20 {\scriptsize$\pm$ 0.00} & 0.54 {\scriptsize$\pm$ 0.00} \\
SAFE & 0.66 {\scriptsize$\pm$ 0.01} & \cellcolor{deltas}+0.09 & 0.18 {\scriptsize$\pm$ 0.00} & 0.50 {\scriptsize$\pm$ 0.01} \\
OpenScholar + S2 & 0.45 {\scriptsize$\pm$ 0.01} & \cellcolor{deltaxl}+0.31 & 0.23 {\scriptsize$\pm$ 0.00} & 0.41 {\scriptsize$\pm$ 0.03} \\
\midrule
\textbf{ProClaim} (ours) & \underline{0.75} {\scriptsize$\pm$ 0.01} & -- & \underline{0.14} {\scriptsize$\pm$ 0.00} & 0.38 {\scriptsize$\pm$ 0.01} \\
\bottomrule
\end{tabular}


==> tables/baseline_metrics_main.tex <==
\begin{tabular}{@{} l | *{3}{c} | *{3}{c} @{}}
\toprule
  & \multicolumn{3}{c|}{\cellcolor{headerteal}\textbf{SIGNOR}} & \multicolumn{3}{c}{\cellcolor{headerlavender}\textbf{ConnectomeDB}} \\
\textbf{Method} & Agreement$\uparrow$ & FPR$\downarrow$ & FNR$\downarrow$ & Agreement$\uparrow$ & FPR$\downarrow$ & FNR$\downarrow$ \\
\midrule
Random & 0.33 {\scriptsize$\pm$ 0.01} & 0.33 {\scriptsize$\pm$ 0.01} & 0.65 {\scriptsize$\pm$ 0.01} & 0.34 {\scriptsize$\pm$ 0.01} & 0.33 {\scriptsize$\pm$ 0.00} & 0.64 {\scriptsize$\pm$ 0.02} \\
\midrule
\multicolumn{7}{@{}l}{\textit{LLM Only}} \\[2pt]
Claude Sonnet 4.6 & 0.59 {\scriptsize$\pm$ 0.00} & 0.21 {\scriptsize$\pm$ 0.00} & 0.45 {\scriptsize$\pm$ 0.02} & 0.52 {\scriptsize$\pm$ 0.00} & 0.22 {\scriptsize$\pm$ 0.00} & 0.47 {\scriptsize$\pm$ 0.00} \\
Gemini 2.5 Flash & 0.59 {\scriptsize$\pm$ 0.00} & 0.21 {\scriptsize$\pm$ 0.00} & 0.42 {\scriptsize$\pm$ 0.00} & 0.57 {\scriptsize$\pm$ 0.00} & 0.22 {\scriptsize$\pm$ 0.00} & 0.43 {\scriptsize$\pm$ 0.01} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Static Retrieval S2 Top 5}} \\[2pt]
Claude Sonnet 4.6 & 0.67 {\scriptsize$\pm$ 0.00} & 0.23 {\scriptsize$\pm$ 0.00} & 0.47 {\scriptsize$\pm$ 0.00} & 0.46 {\scriptsize$\pm$ 0.00} & 0.27 {\scriptsize$\pm$ 0.00} & 0.63 {\scriptsize$\pm$ 0.00} \\
Gemini 2.5 Flash & 0.65 {\scriptsize$\pm$ 0.00} & 0.27 {\scriptsize$\pm$ 0.00} & 0.50 {\scriptsize$\pm$ 0.00} & 0.49 {\scriptsize$\pm$ 0.00} & 0.28 {\scriptsize$\pm$ 0.00} & 0.62 {\scriptsize$\pm$ 0.00} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Static Retrieval Web Top 5}} \\[2pt]
Claude Sonnet 4.6 & 0.68 {\scriptsize$\pm$ 0.01} & 0.21 {\scriptsize$\pm$ 0.00} & 0.55 {\scriptsize$\pm$ 0.03} & 0.44 {\scriptsize$\pm$ 0.01} & 0.25 {\scriptsize$\pm$ 0.00} & 0.65 {\scriptsize$\pm$ 0.01} \\
Gemini 2.5 Flash & 0.65 {\scriptsize$\pm$ 0.02} & 0.24 {\scriptsize$\pm$ 0.01} & 0.58 {\scriptsize$\pm$ 0.01} & 0.55 {\scriptsize$\pm$ 0.00} & 0.24 {\scriptsize$\pm$ 0.00} & 0.60 {\scriptsize$\pm$ 0.00} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Adaptive Retrieval}} \\[2pt]
ReAct + S2 & 0.62 {\scriptsize$\pm$ 0.03} & 0.20 {\scriptsize$\pm$ 0.01} & 0.47 {\scriptsize$\pm$ 0.04} & 0.62 {\scriptsize$\pm$ 0.01} & 0.18 {\scriptsize$\pm$ 0.00} & 0.43 {\scriptsize$\pm$ 0.01} \\
ReAct + Web & 0.70 {\scriptsize$\pm$ 0.01} & 0.17 {\scriptsize$\pm$ 0.00} & 0.47 {\scriptsize$\pm$ 0.04} & 0.68 {\scriptsize$\pm$ 0.00} & 0.16 {\scriptsize$\pm$ 0.00} & \underline{0.26} {\scriptsize$\pm$ 0.02} \\
FIRE & 0.72 {\scriptsize$\pm$ 0.01} & 0.18 {\scriptsize$\pm$ 0.00} & 0.51 {\scriptsize$\pm$ 0.02} & 0.59 {\scriptsize$\pm$ 0.00} & 0.21 {\scriptsize$\pm$ 0.00} & 0.55 {\scriptsize$\pm$ 0.01} \\
SAFE & 0.71 {\scriptsize$\pm$ 0.01} & 0.18 {\scriptsize$\pm$ 0.01} & 0.49 {\scriptsize$\pm$ 0.03} & 0.64 {\scriptsize$\pm$ 0.01} & 0.18 {\scriptsize$\pm$ 0.00} & 0.51 {\scriptsize$\pm$ 0.01} \\
OpenScholar + S2 & 0.40 {\scriptsize$\pm$ 0.01} & 0.24 {\scriptsize$\pm$ 0.01} & 0.45 {\scriptsize$\pm$ 0.02} & 0.46 {\scriptsize$\pm$ 0.01} & 0.22 {\scriptsize$\pm$ 0.00} & 0.39 {\scriptsize$\pm$ 0.03} \\
\midrule
\textbf{ProClaim} (ours) & \underline{0.76} {\scriptsize$\pm$ 0.01} & \underline{0.13} {\scriptsize$\pm$ 0.01} & \underline{0.37} {\scriptsize$\pm$ 0.03} & \underline{0.75} {\scriptsize$\pm$ 0.01} & \underline{0.14} {\scriptsize$\pm$ 0.00} & 0.39 {\scriptsize$\pm$ 0.00} \\
\bottomrule
\end{tabular}


==> tables/iclr_budget.tex <==
% \begin{tabular}{@{} l c c c c c @{}}
% \toprule
% \textbf{Method} & SIGNOR & ConnectomeDB & ExTRI & NUBASE & NASA \\
% \midrule
% \multicolumn{6}{@{}l}{\textit{LLM Only}} \\[2pt]
% Claude Sonnet 4.6 & none & none & none & none & none \\
% Gemini 2.5 Flash & none & none & none & none & none \\
% \midrule
% \multicolumn{6}{@{}l}{\textit{Static Retrieval, S2 Top 5}} \\[2pt]
% Claude Sonnet 4.6 & 1 search & 1 search & 1 search & 1 search & 1 search \\
% Gemini 2.5 Flash & 1 search & 1 search & 1 search & 1 search & 1 search \\
% \midrule
% \multicolumn{6}{@{}l}{\textit{Adaptive Retrieval}} \\[2pt]
% ReAct & 20 steps & 20 steps & 20 steps & 20 steps & 20 steps \\
% FIRE & 20 steps & 20 steps & 20 steps & 20 steps & 20 steps \\
% SAFE & 20 steps & 20 steps & 20 steps & 20 steps & 20 steps \\
% OpenScholar & 25 steps & 25 steps & 25 steps & 25 steps & 25 steps \\
% \midrule
% \multicolumn{6}{@{}l}{\textit{General-Purpose Agents}} \\[2pt]
% Claude Code & uncapped & uncapped & uncapped & uncapped & uncapped \\
% Codex & uncapped & uncapped & - & - & - \\
% \midrule
% \textbf{ProClaim} & judge, $\leq$4 rounds & judge, $\leq$4 rounds & judge, $\leq$4 rounds & judge, $\leq$4 rounds & judge, $\leq$4 rounds \\
% \bottomrule
% \end{tabular}


==> tables/iclr_doc_guided.tex <==
% \begin{tabular}{@{} l | c c c | c c c | c c c @{}}
% \toprule
%  & \multicolumn{3}{c}{\textbf{SIGNOR}} & \multicolumn{3}{c}{\textbf{ConnectomeDB}} & \multicolumn{3}{c}{\textbf{Both}} \\
% \textbf{Setting} & Agr.$\uparrow$ & Abst. & S$\to$R & Agr.$\uparrow$ & Abst. & S$\to$R & Agr.$\uparrow$ & Abst. & S$\to$R \\
% \midrule
% Document-guided & 0.65 & 0.22 & 0.32 & 0.59 & 0.20 & 0.24 & 0.60 & 0.20 & 0.26 \\
% Static retrieval & 0.66 & 0.10 & 0.63 & 0.48 & 0.12 & 0.65 & 0.52 & 0.12 & 0.64 \\
% \midrule
% ProClaim & 0.78 & 0.10 & 0.11 & 0.76 & 0.09 & 0.11 & 0.76 & 0.09 & 0.11 \\
% \bottomrule
% \end{tabular}


==> tables/iclr_evidence_state.tex <==
\begin{tabular}{@{} l | c c | c c | c c | c c | c c @{}}
\toprule
 & \multicolumn{2}{c}{\textbf{SIGNOR}} & \multicolumn{2}{c}{\textbf{ConnectomeDB}} & \multicolumn{2}{c}{\textbf{ExTRI}} & \multicolumn{2}{c}{\textbf{NUBASE}} & \multicolumn{2}{c}{\textbf{NASA}} \\
\textbf{System} & Agr.$\uparrow$ & Abst. & Agr.$\uparrow$ & Abst. & Agr.$\uparrow$ & Abst. & Agr.$\uparrow$ & Abst. & Agr.$\uparrow$ & Abst. \\
\midrule
ReAct, 10 steps & 0.69 & 0.20 & 0.62 & 0.22 & - & - & - & - & - & - \\
ReAct, 20 steps & 0.78 & 0.10 & 0.70 & 0.08 & 0.74 & 0.16 & 0.18 & 0.71 & 0.55 & 0.39 \\
ReAct, 40 steps & 0.79 & 0.05 & 0.73 & 0.07 & - & - & - & - & - & - \\
\midrule
ProClaim & 0.80 & 0.12 & 0.78 & 0.05 & 0.72 & 0.14 & 0.52 & 0.36 & 0.66 & 0.14 \\
\bottomrule
\end{tabular}


==> tables/iclr_judge.tex <==
\begin{tabular}{@{} l | c c c | c c c | c c c | c c c | c c c @{}}
\toprule
 & \multicolumn{3}{c}{\textbf{SIGNOR}} & \multicolumn{3}{c}{\textbf{ConnectomeDB}} & \multicolumn{3}{c}{\textbf{ExTRI}} & \multicolumn{3}{c}{\textbf{NUBASE}} & \multicolumn{3}{c}{\textbf{NASA}} \\
\textbf{Judge} & Agr. & Abst. & Iter. & Agr. & Abst. & Iter. & Agr. & Abst. & Iter. & Agr. & Abst. & Iter. & Agr. & Abst. & Iter. \\
\midrule
\multicolumn{16}{@{}l}{\textit{Stopping rules that ignore the evidence state}} \\[2pt]
Fixed rounds & 0.69 & 0.18 & 3.36 & 0.60 & 0.26 & 3.30 & - & - & - & - & - & - & - & - & - \\
Constant insufficient & 0.79 & 0.11 & 2.64 & 0.67 & 0.15 & 3.18 & - & - & - & - & - & - & - & - & - \\
Random signal & 0.76 & 0.17 & 3.11 & 0.74 & 0.11 & 3.20 & - & - & - & - & - & - & - & - & - \\
\midrule
\multicolumn{16}{@{}l}{\textit{Off-the-shelf LLM judges}} \\[2pt]
Qwen3.5 9B & 0.71 & 0.18 & 2.63 & 0.75 & 0.09 & 2.73 & - & - & - & - & - & - & - & - & - \\
Claude Haiku 4.5 & 0.76 & 0.11 & 2.48 & 0.75 & 0.07 & 2.36 & - & - & - & - & - & - & - & - & - \\
Claude Sonnet 4.6 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\midrule
\multicolumn{16}{@{}l}{\textit{Trained judge}} \\[2pt]
Trained judge & 0.80 & 0.12 & 3.21 & 0.78 & 0.05 & 2.87 & 0.72 & 0.14 & 2.95 & - & - & - & 0.66 & 0.14 & 2.35 \\
\bottomrule
\end{tabular}


==> tables/iclr_judge_complete.tex <==
\begin{tabular}{@{} l | c c c | c c c @{}}
\toprule
 & \multicolumn{3}{c}{\textbf{SIGNOR}} & \multicolumn{3}{c}{\textbf{ConnectomeDB}} \\
\textbf{Judge} & Agr. & Abst. & Iter. & Agr. & Abst. & Iter. \\
\midrule
\multicolumn{7}{@{}l}{\textit{Stopping rules that ignore the evidence state}} \\[2pt]
Fixed rounds & 0.69 & 0.18 & 3.36 & 0.60 & 0.26 & 3.30 \\
Constant insufficient & 0.79 & 0.11 & 2.64 & 0.67 & 0.15 & 3.18 \\
Random signal & 0.76 & 0.17 & 3.11 & 0.74 & 0.11 & 3.20 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Off-the-shelf LLM judges}} \\[2pt]
Qwen3.5 9B & 0.71 & 0.18 & 2.63 & 0.75 & 0.09 & 2.73 \\
Claude Haiku 4.5 & 0.76 & 0.11 & 2.48 & 0.75 & 0.07 & 2.36 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Trained judge}} \\[2pt]
Trained judge & 0.80 & 0.12 & 3.21 & 0.78 & 0.05 & 2.87 \\
\bottomrule
\end{tabular}

